Return-Based Contrastive Representation Learning for Reinforcement Learning

Recently, various auxiliary tasks have been proposed to accelerate representation learning and improve sample efficiency in deep reinforcement learning (RL). However, existing auxiliary tasks do not take the characteristics of RL problems into consideration and are unsupervised. By leveraging returns, the most important feedback signals in RL, we propose a novel auxiliary task that forces the learnt representations to discriminate state-action pairs with different returns. Our auxiliary loss is theoretically justified to learn representations that capture the structure of a new form of state-action abstraction, under which state-action pairs with similar return distributions are aggregated together. In low data regime, our algorithm outperforms strong baselines on complex tasks in Atari games and DeepMind Control suite, and achieves even better performance when combined with existing auxiliary tasks.

==> DMC_table.tex <==
% \begin{table*}[ht]
% \small
% \centering
% \begin{tabular}{cccccc}
% \toprule
% 500K STEP SCORES & Our CURL & CURL (Paper) & DREAMER & SAC+AE & State SAC\\
% \midrule
% FINGER, SPIN & $828 \pm 137$ & $\mathbf{926 \pm 45}$ & $796  \pm 183$  & $884  \pm 128$ &  $923 \pm 21$ \\
% CARTPOLE, SWINGUP & $808 \pm 39$ &  $\mathbf{841 \pm 45} $&  $ 762 \pm 27 $ &  $ 735 \pm 63 $ &  $ 848 \pm 15 $\\
% REACHER, EASY & $\mathbf{951 \pm 26}$ & $929 \pm 44$ & $ 793 \pm 164 $ & $ 627 \pm 58 $ & $923 \pm 24 $\\ 
% CHEETAH, RUN  & $526 \pm 59$ & $518 \pm 28$ & $\mathbf{570 \pm 253}$ & $550 \pm 34$ & $795 \pm 30$ \\
% WALKER, WALK & $892 \pm 49$ & $\mathbf{902 \pm 43}$ & $897 \pm 49$ & $847 \pm 48$ & $948 \pm 54 $ \\
% BALL IN CUP, CATCH & $846 \pm 103$ & $\mathbf{959 \pm 27}$ & $879 \pm 87$ & $794 \pm 58$ & $974 \pm 33$ \\
% % \bottomrule
% \midrule
% 100K STEP SCORES & Our CURL & CURL (Paper) & DREAMER & SAC+AE & State SAC\\
% \midrule
% FINGER, SPIN & $749 \pm 138$ & $ \mathbf{767 \pm 56}$ &  $341 \pm 70$ &  $740 \pm 64$ & $811 \pm 46$ \\
% CARTPOLE, SWINGUP & $367 \pm 74$ &  $\mathbf{582 \pm 146} $ &  $326 \pm 27$ &  $311 \pm 11$ &  $835 \pm 22$\\
% REACHER, EASY & $\mathbf{576 \pm 88}$ & $ 538 \pm 233 $ &  $314 \pm 155$ &  $274 \pm 14$ & $ 746 \pm 25 $\\ 
% CHEETAH, RUN  & $225 \pm 32$ & $ \mathbf{299 \pm 48} $ &  $ 235 \pm 137$ &  $ 267 \pm 24 $ & $616 \pm 18$ \\
% WALKER, WALK & $ \mathbf{410 \pm 86} $ & $ 403 \pm 24 $ & $ 277 \pm 12$ & $394 \pm 22$ & $891 \pm 82$ \\
% BALL IN CUP, CATCH & $546 \pm 210 $ & $ \mathbf{769 \pm 43} $ &  $246 \pm 174$ &  $391 \pm 82$ &  $746 \pm 91$ \\
% \bottomrule
% \end{tabular}
% \caption{
% Scores achieved by RCRL and other baseline algorithms on DMControl-500k and DMControl-100k.
% We show the mean and the standard deviation over five random seeds.
% }
% \label{tab:dmc}
% \end{table*}

==> experiment.tex <==
Key idea (ordered by the priority): 
\begin{itemize}
  \item Evaluation: CURL $<$ CURL + RCRL (CURL $<$ RCRL).
  \item Analysis: NTK and cosine distance of $\phi(s,a)$ (on both postive and negative pairs).
  \item Ablation: different ways to choose negative samples.

\end{itemize}

% Enhance CURL across all their used benchmarks.
\subsection{Evaluation}

In this section, we evaluate our method on two commonly used benchmarks: \textbf{DMControl Suite}~\citep{tassa2020dmcontrol} and \textbf{Atari 2600 Games}~\citep{bellemare2013arcade}. 


\subsubsection{DMControl Suite}

\textbf{Metric:} DMControl-500k, DMControl-100k\footnote{environment steps}. 


\begin{table*}[ht]
\small
\centering
\begin{tabular}{cccccc}
\toprule
500K STEP SCORES & Our CURL & CURL (Paper) & DREAMER & SAC+AE & State SAC\\
\midrule
FINGER, SPIN & $828 \pm 137$ & $\mathbf{926 \pm 45}$ & $796  \pm 183$  & $884  \pm 128$ &  $923 \pm 21$ \\
CARTPOLE, SWINGUP & $808 \pm 39$ &  $\mathbf{841 \pm 45} $&  $ 762 \pm 27 $ &  $ 735 \pm 63 $ &  $ 848 \pm 15 $\\
REACHER, EASY & $\mathbf{951 \pm 26}$ & $929 \pm 44$ & $ 793 \pm 164 $ & $ 627 \pm 58 $ & $923 \pm 24 $\\ 
CHEETAH, RUN  & $526 \pm 59$ & $518 \pm 28$ & $\mathbf{570 \pm 253}$ & $550 \pm 34$ & $795 \pm 30$ \\
WALKER, WALK & $892 \pm 49$ & $\mathbf{902 \pm 43}$ & $897 \pm 49$ & $847 \pm 48$ & $948 \pm 54 $ \\
BALL IN CUP, CATCH & $846 \pm 103$ & $\mathbf{959 \pm 27}$ & $879 \pm 87$ & $794 \pm 58$ & $974 \pm 33$ \\
% \bottomrule
\midrule
100K STEP SCORES & Our CURL & CURL (Paper) & DREAMER & SAC+AE & State SAC\\
\midrule
FINGER, SPIN & $749 \pm 138$ & $ \mathbf{767 \pm 56}$ &  $341 \pm 70$ &  $740 \pm 64$ & $811 \pm 46$ \\
CARTPOLE, SWINGUP & $367 \pm 74$ &  $\mathbf{582 \pm 146} $ &  $326 \pm 27$ &  $311 \pm 11$ &  $835 \pm 22$\\
REACHER, EASY & $\mathbf{576 \pm 88}$ & $ 538 \pm 233 $ &  $314 \pm 155$ &  $274 \pm 14$ & $ 746 \pm 25 $\\ 
CHEETAH, RUN  & $225 \pm 32$ & $ \mathbf{299 \pm 48} $ &  $ 235 \pm 137$ &  $ 267 \pm 24 $ & $616 \pm 18$ \\
WALKER, WALK & $ \mathbf{410 \pm 86} $ & $ 403 \pm 24 $ & $ 277 \pm 12$ & $394 \pm 22$ & $891 \pm 82$ \\
BALL IN CUP, CATCH & $546 \pm 210 $ & $ \mathbf{769 \pm 43} $ &  $246 \pm 174$ &  $391 \pm 82$ &  $746 \pm 91$ \\
\bottomrule
\end{tabular}
\caption{Scores achieved by SCRL (mean \& standard deviation for 5 seeds) and baselines on DMControl-500k and DMControl-100k.}\label{tab:main exp table}
\end{table*}


% \textbf{Backup Metric}: Trainig Curves of DMControl. 


\subsubsection{Atari 2600 Games}

\textbf{Metric}: Atari-100K

% \textbf{Backup Metric}: Train Longer

\begin{table*}[!htb]
\centering
\tiny
\begin{tabular}{lcccccccc}
\toprule
GAME & HUMAN  & RAINBOW & SIMPLE & OTRAINBOW & EFF. RAINBOW & CURL & Our CURL & RCRL \\
\midrule
ALIEN & $7127.7$ & $318.7$ & $616.9$ & $824.7$ & $739.9$ & $558.2$&$\mathbf{ 847.4}$ \\
AMIDAR & 1719.5  & 32.5 & 88.0 & 82.8 & $\mathbf{188.6}$ & 142.1 & 168.0 \\
ASSAULT & 742.0  & 231 & 527.2 & 351.9 & 431.2 & 600.6  & $\mathbf{606.8}$\\
ASTERIX & 8503.3  & 243.6 & $\mathbf{1128.3}$ & 628.5 & 470.8 & 734.5 &629.0 \\
BANK HEIST & 753.1  & 15.55 & 34.2 & $\mathbf{182.1}$ & 51.0 & 131.6 & 176.6\\
BATTLE ZONE & 37187.5  & 2360.0 & 5184.4 & 4060.6 & 10124.6 & 14870.0& $\mathbf{21820.0}$ \\
BOXING & 12.1  & -24.8 & $\mathbf{9 . 1}$ & 2.5 & 0.2 & 1.2 &3.5 \\
BREAKOUT & 30.5  & 1.2 & $\mathbf{1 6 . 4}$ & 9.84 & 1.9 & 4.9 &3.5\\
CHOPPER COMMAND & 7387.8 & 120.0 & $\mathbf{1 2 4 6 . 9}$ & 1033.33 & 861.8 & 1058.5 & 1096.0 \\
CRAZY\_CLIMBER & 35829.4  & 2254.5 & $\mathbf{6 2 5 8 3 . 6}$ & 21327.8 & 16185.3 & 12146.5&19420.0 \\
DEMON\_ATTACK & 1971.0  & 163.6 & 208.1 & 711.8 & 508.0 & 817.6&$\mathbf{860.8}$ \\
FREEWAY & 29.6 & 0.0 & 20.3 & 25.0 & $27.9$ & 26.7&$\mathbf{28.6}$ \\
FROSTBITE & 4334.7  & 60.2 & 254.7 & 231.6 & 866.8 & 1181.3&$\mathbf{2154.8}$ \\
GOPHER & 2412.5  & 431.2 & 771.0 & $\mathbf{7 7 8 . 0}$ & 349.5 & 669.3 & 426.4 \\
HERO & 30826.4  & 487 & 2656.6 & 6458.8 & 6857.0 & 6279.3& $\mathbf{6884.9}$ \\
JAMESBOND & 302.8  & 47.4 & 125.3 & 112.3 & 301.6 & $\mathbf{4 7 1 . 0}$ &368.0\\
KANGAROO & 3035.0  & 0.0 & 323.1 & 605.4 & 779.3 & 872.5 &$\mathbf{1410.0}$ \\
KRULL & 2665.5  & 1468 & $\mathbf{4 5 3 9 . 9}$ & 3277.9 & 2851.5 & 4229.6 &2928.9\\
KUNG\_FU\_MASTER & 22736.3  & $0 .$ & $\mathbf{1 7 2 5 7 . 2}$ & 5722.2 & 14346.1 & 14307.8 & 15804.0 \\
MS\_PACMAN & 6951.6  & 67 & 1480.0 & 941.9 & 1204.1 & 1465.5&$\mathbf{1687.2}$ \\
PONG & 14.6 & -20.6 & $\mathbf{12.8}$ & 1.3 & -19.3 & -16.5 &-16.8\\
PRIVATE EYE & 69571.3  & 0 & 58.3 & 100.0 & 97.8 &218.4 &$\mathbf{293.4}$ \\
QBERT & 13455.0 & 123.46 & $\mathbf{1 2 8 8 . 8}$ & 509.3 & 1152.9 & 1042.4 & 1272.5 \\
ROAD\_RUNNER & 7845.0 & 1588.46 & 5640.6 & 2696.7 & $\mathbf{9 6 0 0 . 0}$ & 5661.0 & 8890.0 \\
SEAQUEST & 42054.7  & 131.69 & $\mathbf{6 8 3 . 3}$ & 286.92 & 354.1 & 384.5 & 444.4 \\
UP\_N\_DOWN & 11693.2  & 504.6 & 3350.3 & 2847.6 & 2877.4 & 2955.2&$\mathbf{3475.6}$ \\
\midrule
Median HNS & $100.0\%$ & $0.0\%$ & $14.4\%$ &$20.4\%$ & $16.1\%$ & $17.5\%$ & $17.99\%$ &  $16.35\%$ \\
\bottomrule
\end{tabular}
\caption{Results of our method and baselines on 26 environments from Atari 2600 Games at 100k timesteps. }
\vspace{-0.3cm}
\label{tab:atari}
\end{table*}

We need some powerful sentences here to highlight our strong performance, for example, CURL outperforms prior pixel-based methods, both model-based and model-free, on complex tasks in the DeepMind Control Suite and Atari
Games showing 1.9x and 1.2x performance gains
at the 100K environment and interaction steps
benchmarks respectively (from CURL). 

\subsection{Analysis on Learned Representations}


\subsection{Ablation Study on the Choices of Negative Samples}















==> iclr2021_description_backup.tex <==
\section{Submission of conference papers to ICLR 2021}

ICLR requires electronic submissions, processed by
\url{https://openreview.net/}. See ICLR's website for more instructions.

If your paper is ultimately accepted, the statement {\tt
  {\textbackslash}iclrfinalcopy} should be inserted to adjust the
format to the camera ready requirements.

The format for the submissions is a variant of the NeurIPS format.
Please read carefully the instructions below, and follow them
faithfully.

\subsection{Style}

Papers to be submitted to ICLR 2021 must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the ICLR \LaTeX{} style files obtainable at the
ICLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for ICLR and other conference information are available online at:
\begin{center}
  \url{http://www.iclr.cc/}
\end{center}
The file \verb+iclr2021_conference.pdf+ contains these
instructions and illustrates the
various formatting requirements your ICLR paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+iclr2021_conference.sty+ and \verb+iclr2021_conference.bst+ (to be used with \LaTeX{}2e). The file
\verb+iclr2021_conference.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in small caps and left-aligned.
All pages should start at 1~inch (6~picas) from the top of the page.

Authors' names are
set in boldface, and each name is placed above its corresponding
address. The lead author's name is to be listed first, and
the co-authors' names are set to follow. Authors sharing the
same address can be on the same line.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.


There will be a strict upper limit of 8 pages for the main text of the initial submission, with unlimited additional pages for citations. Note that the upper page limit differs from last year!Authors may use as many pages of appendices (after the bibliography) as they wish, but reviewers are not required to read these. During the rebuttal phase and for the camera ready version, authors are allowed one additional page for the main text, for a strict upper limit of 9 pages.

\section{Headings: first level}
\label{headings}

First level headings are in small caps,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in small caps,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in small caps,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
  \usepackage[dvips]{graphicx} ...
  \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
  \usepackage[pdftex]{graphicx} ...
  \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

\subsubsection*{Author Contributions}
If you'd like to, you may include  a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.

==> related_work.tex <==
\subsection{State abstraction}

\textbf{Definitions of abstractions.}
Aggregating states or state abstraction \citep{li2006towards} can increase sample efficiency in RL (empirically demonstrated by \cite{abel2016near}). 
There are different levels of abstractions, 
such as homomorphism \citep{ravindran2003smdp,ravindran2004algebraic}, bisimulation \citep{dean1997model,givan2003equivalence}, $Q^\pi$ irrelevance, $Q^*$ irrelevance, $a^*$-irrelevance, and $\pi^*$ irrelevance \citep{li2006towards}, arranged from finest to coarsest.

\textbf{Properties of abstractions.}
People investigate approximate form of different abstractions and how they can be used to bound optimality (i.e., whether abstract MDP permits an optimal solution) \citep{abel2016near,jiang2018notes}.
People also investigate whether different forms of abstractions secure Q-learning: 
It is shown that $Q^*$ irrelevance (with a gap assumption) secures Q-learning \citep{li2009unifying,abel2016near}, but Q-learning may break down for $\pi^*$ irrelevance \citep{jong2005state}.

\textbf{Finer or coarser.}
Although finer abstractions lead to lower approximation error, coarser abstractions result in lower estimation error \citep{jiang2015abstraction}, which may be more efficient
\footnote{It is shown that the MSE between $V^*$ and the value of the optimal policy on the abstracted MDP can be written as an addition of an approximation error and an estimation error (since the abstraction is estimated based on a dataset).}.
Moreover, it is shown that finding an bisimulation (even if it exists) requires a number of samples that is exponential in horizon (see Proposition B.1 in \cite{modi2020sample}).
% In terms of Q-learning, it is shown that (approximate) $Q^*$ irrelevance secures Q-learning \citep{li2009unifying,abel2016near}, but Q-learning may break down for $\pi^*$ irrelevance \citep{jong2005state}.
% \footnote{We can demonstrate this with an illustration as follows: Efficient RL algorithms depends on the number of states/state-actions. We can also prove that the number of abstractions for policy irrelevance is no more than that of bisimulation and homomorphism.}.
% ), as long as the abstraction preserves the optimal properties (such as optimal Q values or optimal policies).

\textbf{From abstraction to metric/representation.}
Similar to bisimulation metric \citep{ferns2004metrics,ferns2011bisimulation} that is proposed to associate bisimulation, 
we propose to a $Q^\pi$ irrelevance metric related to the coarser form of abstraction, $Q^\pi$ irrelevance.

\textbf{State-action abstraction.}
Few authors investigate state-action abstractions: homomorphism \cite{ravindran2003smdp} deals with action aggregation and permutation. \cite{maillard2020upper} and \cite{biza2018online} define a state-action based homomorphism.
Here, we study a new form of state-action abstraction (which is similar to $Q^\pi$ irrelevance).
% Moreover, although previous work propose to define abstraction over state-actions instead of states \citep{maillard2020upper}, we study a new form of state-action abstraction (which is similar to $Q^\pi$ irrelevance).

\textbf{Abstraction algorithms.}
In terms of how to obtain abstractions, authors focus on learning a representation associated with bisimulation \citep{ruan2015representation,gelada2019deepmdp,zhang2020learning,van2020mdp}, homomorphism \citep{biza2018online} or $\phi_{a^*}$-irrelevance \citep{jong2005state}.
Particularly, \cite{ortner2013adaptive} use a UCRL algorithm \citep{auer2009near} to quantify the similarity between two states in terms of reward and transition, and further aggregate the states.
DeepMDP \citep{gelada2019deepmdp} and DBC \citep{zhang2020learning} include experiments on complex tasks such as Atari or DMControl and achieve good performance.

% Previous work closely related to ours is the one tries to learn a representation of a policy irrelevance abstraction. 

\subsection{Auxiliary task}

In reinforcement learning, the auxiliary-task first proposed by \cite{sutton2011horde} can improve sample efficiency. 

\textbf{Model-based setting/world model.}
In the model-based settings, world models can be used as auxiliary tasks and lead to better performance, such as CRAR \citep{franccois2019combined}, Dreamer \citep{hafner2019dream} and PlaNet \citep{hafner2019learning}. 
These papers learn latent representations of the state end-to-end which can be regarded as aggregating the states implicitly. 
However, such methods are unstable to train and relies on regularizations to converge.

\textbf{Model-free setting.}
In the model-free settings, many algorithms construct various auxiliary tasks to improve performance, such as predicting the future states \citep{guo2020bootstrap,jaderberg2016reinforcement}, recognizing from different transformations to the image-based states \citep{srinivas2020curl}, or combination of different auxiliary objectives that aid representation learning \citep{de2018integrating}.
The most relevant work focus on predicting various value functions:
\cite{veeriah2019discovery} predict value functions with different cumulants, \cite{schaul2015universal} and \cite{borsa2018universal} learn value functions with different goals or rewards.
AVF \citep{bellemare2019geometric} and value improvement path \citep{dabney2020value}
predict value functions under different policies, which are similar to ours.
However, we justify such auxiliary tasks through the lens of state abstraction instead of a geometric view which only works when the values are linear combinations of the representation. 
Also, our algorithm is much simpler than AVF with only an auxiliary loss in addition to DQN based algorithms.
PastPolicies and PastMixture in \cite{dabney2020value} use auxiliary tasks based on bootstrapping old Q functions or Q functions learned with different learning rates, which is regression based on moving targets.
We design auxiliary tasks based on classification towards fixed targets and we may expect this could result in better performance.

% \subsection{Miscellany}



==> related_work_backup.tex <==

\section{Related Works}
\subsection{Fundamentals}
% 1.~\textbf{Soft State Aggregation}: Reinforcement learning with soft state aggregation.  Singh, S. P., Jaakkola, T., and Jordan, M. I. NIPS 1995.

% 6.~\textbf{Discovery by Bisimulation Metrics}: Basis function discovery using spectral clustering and bisimulation metrics. Comanici, G. and Precup, D. In AAMAS 2011. 

% 8.~\textbf{SMDP Homomorphisms}: SMDP homomorphisms: An algebraic approach to abstraction in semi-Markov decision processes. Balaraman Ravindran and Andrew G. Barto. In IJCAI-03. 2003.  

% 11.~\textbf{Policy Irrelevance}: Nicholas K. Jong and Peter Stone. State abstraction discovery from irrelevant state variables. In IJCAI-05, 2005.  


\begin{itemize}
\item \textbf{Bisimulation}: Equivalence notions and model minimization in Markov decision processes. Robert Givan, Thomas Dean, and Matthew Greig. Artificial Intelligence. 2003.

\item \textbf{Approximate Bisimulation}: Model reduction techniques for computing approximately optimal solutions for Markov decision processes. Thomas Dean, Robert Givan, and Sonia M.Leach. UAI-97.  

\item \textbf{Bisimulation Metrics}: Metrics for finite Markov decision processes. Norm Ferns, Prakash Panangaden, and Doina Precup. In Proceedings of the Twentieth Conference on Uncertainty in Artificial Intelligence (UAI-04). 2004.

\item \textbf{Bisimulation Metrics}: Bisimulation metrics for continuous markov decision processes. Ferns, N., Panangaden, P., and Precup, D. 2011.

\item \textbf{MDP Homomorphisms}: An algebraic approach to abstraction in reinforcement learning. Balaraman Ravindran. Phd Thesis. 2004.

\item \textbf{Approximate MDP Homomorphisms}: Approximate Homomorphisms: A Framework for Non-Exact Minimization in Markov Decision Processes. Balaraman Ravindran and Andrew G. Barto. In International Conference on Knowledge Based Computer Systems. 2004. 

\item \textbf{MDP Homomorphisms Metrics}: Bounding Performance Loss in Approximate MDP Homomorphisms. NIPS 2008.

\item \textbf{Towards a Unified Theory of State Abstraction for MDPs}. Lihong li, et al. 2006.  

\end{itemize}

\subsection{Advances}
% 2.~Representation Discovery in Sequential Decision Making. AAAI 2010. 

% 3.~Representation discovery for mdps using bisimulation metrics. AAAI 2015.

% 4.~Abstraction selection in model-based reinforcement learning. Jiang, N., Kulesza, A., and Singh, S. In International Conference on Machine Learning, pp. 179–188, 2015.

% 5.~Near optimal behavior via approximate state abstraction. Abel, D., Hershkowitz, D. E., and Littman, M. L. arXiv. 2017.

% 6.~Online Abstraction with MDP Homomorphisms
% for Deep Learning. AAMAS 2019. 

% 7.~Soft State Aggregation: State Aggregation Learning from Markov Transition Data. NeurlPS 2019. 

% 9.~Combined Reinforcement Learning via Abstract Representations. Vincent François-Lavet, Yoshua Bengio, Doina Precup, Joelle Pineau. AAAI 2019. 


% 15. Integrating State Representation Learning into Deep Reinforcement Learning. ICRA 2018.

% 16.~\textbf{Structured representations}: Deep reinforcement learning with relational inductive biases. ICLR 2019. 


\begin{itemize}
    \item \textbf{Value Function Geometry}: Proto-value functions A laplacian framework for learning representation and control in markov decision processes. Journal of Machine Learning Research. Mahadevan, S. and Maggioni, M. 2007.
    \item \textbf{Value Function Geometry}: 
    A geometric perspective on optimal representations for reinforcement learning. Bellemare, M. G., et al. ICML 2019.
    \item \textbf{Value Function Geometry}: 
    The Value-Improvement Path Towards Better Representations for Reinforcement Learning. Deepmind. arXiv 2020.
    \item \textbf{Auxiliary Loss}:
    Reinforcement learning with unsupervised auxiliary tasks. Jaderberg, M., Mnih, V., Czarnecki, W. M., Schaul, T., Leibo, J. Z., Silver, D., and Kavukcuoglu, K. In International Conference on Learning Representations (ICLR), 2017.
    \item \textbf{Auxiliary Loss}:
    DeepMDP: Learning Continuous Latent Space Models for Representation Learning. ICML 2019.
    \item \textbf{Auxiliary Loss}:
    Learning Invariant Representations for Reinforcement Learning without Reconstruction. Zhang A, McAllister R, Calandra R, et al. arXiv preprint arXiv:2006.10742, 2020. 
    \item \textbf{MDP Homomorphisms Metrics Loss}:
    Plannable Approximations to MDP Homomorphisms: Equivariance under Actions. Elise van der Pol, Thomas Kipf, Frans A. Oliehoek, Max Welling. AAMAS 2020. 
    \item \textbf{Alternating SRL and RL}: Integrating State Representation Learning into Deep Reinforcement Learning. ICRA 2018.

\end{itemize}

==> theory.tex <==
\subsection{Abstraction and its properties}

This part follows a standard infinite horizon discounted MDP setting/notations. In addition, we use $x\in\mathcal{X}$ to denote the state-actions, i.e., $\mathcal{X} = \mathcal{S} \times \mathcal{A}$. Let $n=|\mathcal{X}|$.

\begin{definition}[$Q$-irrelevance abstraction]
Given a set of policies $\Pi$ and any state-actions $x,\bar{x} \in \mathcal{X}$, 
a $Q$-irrelevance abstraction $\phi_{Q,\Pi}$ is such that $\phi_{Q,\Pi}(x) = \phi_{Q,\Pi}(\bar{x})$ implies $Q^\pi(x)=Q^\pi(\bar{x})$ for any policy $\pi \in \Pi$.
We also define an exact $Q$-irrelevance abstraction $\varphi_{Q,\Pi}$ such that $\varphi_{Q,\Pi}(x) = \varphi_{Q,\Pi}(\bar{x})$ if and only if $Q^\pi(x)=Q^\pi(\bar{x})$ for any policy $\pi \in \Pi$.
\end{definition}

\begin{definition}[\cite{li2006towards}]
Given two abstractions $\phi_1$ and $\phi_2$, we say $\phi_1$ is finer than $\phi_2$, denoted $\phi_1 \succeq \phi_2$, if and only if $\forall x_1, x_2 \in \mathcal{X}, \phi_1(x_1) = \phi_1(x_2)$ implies $\phi_2(x_1) = \phi_2(x_2)$. 
If, in addition, $\phi_1 \neq \phi_2$, then $\phi_1$ is strictly finer than $\phi_2$, denoted $\phi_1 \succ \phi_2$.
We also may say $\phi_2$ is (strictly) coarser than $\phi_1$, denoted $\phi_2 \preceq \phi_1$ ($\phi_2 \prec \phi_1$).
\end{definition}

\begin{remark}
$\phi_{Q,\Pi}$ is the set of abstractions that are finer than $\varphi_{Q,\Pi}$.
% A finer abstraction (such as the identity mapping $\phi_0$) satisfies the definition of $Q$-irrelevance abstraction but does not satisfy the definition of exact $Q$-irrelevance abstraction.
\end{remark}

\begin{definition}[Stationary policies]
The set of all stationary policies is defined as $\Pi_0 = \{\pi \in [0,1]^{\mathcal{S} \times \mathcal{A}} : \sum_{a\in\mathcal{A}}\pi(s,a) = 1\}$. The set of all deterministic stationary policies is defined as 
$\Pi_1 = \{\pi \in \{0,1\}^{\mathcal{S} \times \mathcal{A}} : \sum_{a\in\mathcal{A}}\pi(s,a) = 1\}$.
\end{definition}

\begin{lemma}
\label{lemma:detpolicy}
Given $x, \bar{x} \in \mathcal{X}$, if $Q^{\pi_0}(x) \neq Q^{\pi_0}(\bar{x})$ for some ${\pi_0} \in \Pi_0$, there exists $\pi_1 \in \Pi_1$ such that $Q^{\pi_1}(x) \neq Q^{\pi_1}(\bar{x})$.
\end{lemma}

\begin{proof}
Assume $Q^{\pi_0}(x) > Q^{\pi_0}(\bar{x})$ or we can swap $x$ and $\bar{x}$. Let $f(\pi) = Q^\pi(x) - Q^\pi(\bar{x}) = \sum_{s'} \left( p(s'|x) - p(s'|\bar{x}) \right) V^\pi(s') = \delta^T V^\pi$, 
where $\delta \in \mathbb{R}^S$ is a vector, the $s'$-th element of which is $ p(s'|x) - p(s'|\bar{x})$. 
According to Lemma 1 in \cite{bellemare2019geometric}, there exists a deterministic policy $\pi_1$ that maximizes $f(\pi)$. 
Since there exists a (possible stochastic) policy $\pi_0$ such that $f(\pi_0) > 0$, $f(\pi_1) \ge f(\pi_0) > 0$.
Therefore, $Q^{\pi_1}(x) \neq Q^{\pi_1}(\bar{x})$.
\end{proof}

\begin{theorem}
$\varphi_{Q,\Pi_0} = \varphi_{Q,\Pi_1}$.
\end{theorem}

\begin{proof}
Since $\Pi_1 \subset \Pi_0$, $\varphi_{Q,\Pi_0} \succeq \varphi_{Q,\Pi_1}$.
For any $x,\bar{x} \in \mathcal{X}$ such that $\varphi_{Q,\Pi_1}(x) = \varphi_{Q,\Pi_1}(\bar{x})$, $Q^{\pi_1}(x) = Q^{\pi_1}(\bar{x}), \forall \pi_1 \in \Pi_1$. 
Using Lemma \ref{lemma:detpolicy}, this implies that $Q^{\pi_0}(x) = Q^{\pi_0}(\bar{x}), \forall \pi_0 \in \Pi_0$ and therefore $\varphi_{Q,\Pi_0}(x) = \varphi_{Q,\Pi_0}(\bar{x})$, i.e., $\varphi_{Q,\Pi_0} \preceq \varphi_{Q,\Pi_1}$.
\end{proof}

Next we define the corresponding metric and representation of an abstraction.

\begin{definition}[Abstraction metric, \cite{ferns2004metrics}]
Let $\phi$ be an abstraction and $\mathcal{M}$ be the set of all semimetrics on $\mathcal{X}$ that assign distances of at most 1. 
Note that every semimetric $d$ induces an abstraction $\phi_d$, obtained by equating points assigned distance zero by $d$.
We say that $d\in\mathcal{M}$ is an abstraction metric of $\phi$ if $\phi_d=\phi$.
\end{definition}

\begin{remark}
$d(x,\bar{x}) := \mathbb{I}\{\phi(x)\neq \phi(\bar{x})\}$ that assigns distance $0$ if $\phi(x) = \phi(\bar{x})$, otherwise assigns distance $1$, is a simple abstraction metric.
However, this processes no more distinguishing power than $\phi$ and we would like the metric distances vary smoothly.
\end{remark}

\begin{definition}[Abstraction representation]
We say that a state-action representation $\psi: \mathcal{X} \to \mathbb{R}^m$ is an abstraction representation of $\phi$ if: $\psi(x) = \psi(\bar{x})$ if and only if $\phi(x) = \phi(\bar{x})$, where $m$ is the dimension of the representation.
\end{definition}

\begin{theorem}
Given an abstraction representation $\psi$ of $\phi_{Q, \Pi_0}$ and any policy  $\pi \in \Pi_0$, there exists a function ${Q}: \mathbb{R}^m \to \mathbb{R}$ such that ${Q}({\psi}(x)) = Q^\pi(x), \forall x \in \mathcal{X}$. 
Specifically, there exists ${Q}$ such that ${Q}({\psi}(x)) = Q^*(x), \forall x \in \mathcal{X}$.
\end{theorem}

\begin{proof}
Given a policy $\pi \in \Pi_0$, we can construct a ${Q}$ such that ${Q}({\psi}(x)) = Q^\pi(x), \forall x \in \mathcal{X}$ in the following way:
For all $x\in\mathcal{X}$, one by one, we assign $Q(y) \leftarrow Q^\pi(x)$, where $y = \psi(x)$.
Then, we assign $Q(y)$ with arbitrary values if $y$ does not equal to the representation of any state-actions.
For any $x\in\mathcal{X}$ with $y=\psi(x)$, $Q(y)$ equals either to $Q^\pi(x)$ or $Q^\pi(\bar{x})$ for some other $\bar{x}$ that satisfies $\psi(\bar{x}) = \psi(x)$. However, in the later case, $Q^\pi(x) = Q^\pi(\bar{x})$ since $\psi$ is a state-action representation corresponding to $\phi_{Q, \Pi_0}$.
Therefore, ${Q}({\psi}(x)) = Q^\pi(x), \forall x \in \mathcal{X}$.
This also applies to the optimal policy $\pi^*$.
\end{proof}

The theorem shows that such a state-action representation is fine enough to represent any Q functions. However, to make it complete, we should either 1) prove that any abstraction coarser than $\varphi_{Q, \Pi_0}$ may not preserve Q functions, or at least 2) $\varphi_{Q, \Pi_0}$ is coarser than homomorphism.

\subsection{Algorithm to obtain abstraction}

\begin{assumption}
\label{assumption:detMDP}
We assume a standard tabular case, where the states and actions are discretized. 
We also assume the MDP has deterministic dynamics and a fixed initial state $s_0$.
\end{assumption}

\begin{remark}
Tabular case is a standard setting for MDP analysis. 
Deterministic dynamics and fixed initial state correspond to "no sticky action" and "no random no-op actions at the start" respectively in Atari games.
Determinism is essential to determine the Q values with a single rollout.
\end{remark}

\begin{algorithm}[H]
\label{algo:exact}
\SetAlgoLined
    \KwIn {A set of deterministic policies $\Pi\subseteq \Pi_1$}
    \KwOut {An abstraction metric of $\varphi_{Q, \Pi}$}
    \ForEach{$\pi$ in $\Pi$}{
        Roll out $\pi$ till end and collect the state-actions and the returns $D_\pi = \{(x_i, R_i)\}$
        
        $D \leftarrow D \cup \{(x_i, x_j, y): x_i \in \mathcal{X}, x_j \in \mathcal{X}, y = 1 - \mathbb{I}[ (x_i, R_i) \in D_\pi \text{ \& } (x_j, R_j) \in D_\pi \text{ \& } R_i = R_j ]
        \}
        $
    }
    % $\beta \leftarrow |\Pi| n^2 / |D|$
    
    $d \leftarrow arg \min_{d} L(d;D)$, where \begin{equation}
    \label{eq:loss_d}
    L(d;D) = - \mathbb{E}_{(x_i, x_j, y) \sim D} 
    \left[ 
    y \log d(x_i, x_j) + (1-y) \log ( 1- d(x_i, x_j) )
    % \log \dfrac{d(x_i, x_j)}{1-d(x_i, x_j)} + \beta \log (1-d(x_i, x_k))
    \right] 
    \end{equation} 
    
    \Return{d}
\caption{Learn an abstraction representation of a Q-irrelevance abstraction}
\end{algorithm}

\begin{remark}[Number of steps in one rollout]
Since we assume a discounted setting with infinite horizon, the number of steps in one rollout may be infinite. 
However, we assume there exists an integer $T>0$ and the agent will enter an absorbing state $s_T$ within $T$ steps and receive no more reward from $s_T$.
Therefore, there will be no more than $T$ state-actions in one rollout.
This is a natural extension of the episodic setting to the infinite horizon setting, and is suitable for Atari games.
\end{remark}

\begin{remark}[Stochastic version]
The size of $D$ is $n^2|\Pi|$. 
However, we can perform stochastic gradient update which avoids storing all the transitions.
% However, we can design a stochastic version that uniformly samples state-actions from $\mathcal{X}$ to construct $D$ and use the dataset to perform stochastic gradient update immediately.
\end{remark}

\begin{remark}[Deterministic policies]
Trajectories rolled out by any (possibly stochastic) policy can be considered as being rolled out by a deterministic policy, as long as we choose the same actions from the same states in one trajectory.
% Since we assume the states are fully observable, we do not encounter a same state with different MC returns
% If we do not encounter a same state twice in one rollout, trajectories rolled out by any (possibly stochastic) policy can be considered as being rolled out by a deterministic policy.
\end{remark}

\begin{remark}[Iterating over the state-action space]
We assume that we have access to the state-action space.
% We assume an oracle from where we can uniformly sample from the state-action space.
\end{remark}

Given a set of deterministic policies $\Pi$, although the abstraction $\varphi_{Q,\Pi}$ may be unique, there are more than one abstraction metrics of $\varphi_{Q,\Pi}$. 
We will show that 
the following abstraction metric 1) is a metric of $\varphi_{Q,\Pi}$, and 2) is the metric outputted by Algorithm \ref{algo:exact}.

\begin{equation}
d_1(x_1, x_2) = 1 - \dfrac{\sum_{\pi \in \Pi} \mathbb{I}  [ x_1 \in \mathcal{X}_\pi \text{ \& } x_2 \in \mathcal{X}_\pi \text{ \& } Q^\pi(x_1) = Q^\pi(x_2) ]
}{|\Pi|},
\end{equation}
where $\mathcal{X}_\pi$ is the set of all the state-actions that can be visited starting from $s_0$ and following the policy $\pi$.

\begin{theorem}
% If $\mathcal{X}_\pi = \mathcal{X}$ for any $\pi \in \Pi$, 
$d^*$ is an abstraction metric of $\varphi_{Q, \Pi}$. 
\end{theorem}

\begin{proof}
We can see that $d_1(x_1, x_2)=0$ $\Leftrightarrow$ $x_1$ and $x_2$ have the same Q values for any policy in $\Pi$ $\Leftrightarrow$ $\varphi_{Q,\Pi}(x_1) = \varphi_{Q,\Pi}(x_2)$.
Also, it can be shown that $d_1$ is
a semimetric that assign distances of at most $1$: 
\begin{itemize}
    \item Identity of indiscernibles: $x_1 = x_2 \Rightarrow d_1(x_1, x_2) = 0$;
    \item Symmetry: $d_1(x_1, x_2) = d_1(x_2, x_1)$;
    \item Triangle inequality: $|\Pi|(2 - d_1(x_1, x_2) - d(x_1, x_3)) = \sum_\pi \mathbb{I}[x_1\in\mathcal{X}_\pi \text{ \& } x_2\in\mathcal{X}_\pi \text{ \& } Q^\pi(x_1) = Q^\pi(x_2)] + \mathbb{I}[x_1\in\mathcal{X}_\pi \text{ \& } x_3\in\mathcal{X}_\pi \text{ \& } Q^\pi(x_1) = Q^\pi(x_3)] \le \sum_\pi \mathbb{I}[x_1\in\mathcal{X}_\pi \text{ \& } x_2\in\mathcal{X}_\pi \text{ \& } x_3\in\mathcal{X}_\pi \text{ \& } Q^\pi(x_1) = Q^\pi(x_2) = Q^\pi(x_3)] + |\Pi| \le \sum_\pi \mathbb{I}[x_1\in\mathcal{X}_\pi \text{ \& } x_3\in\mathcal{X}_\pi \text{ \& } Q^\pi(x_1) = Q^\pi(x_3)] + |\Pi| = |\Pi|(2 - d_1(x_1, x_3))$
    \item Boundedness: $0 \le d_1(x_1, x_2) \le 1$;
\end{itemize}
% Identity of indiscernibles and symmetry are easy to verified.
% Triangle inequality can be verified by leveraging the fact that $d(x,y) := \mathbb{I}[x\neq y]$ satisfies triangle inequality.
\end{proof}

% \begin{remark}
% A strange theorem!
% Given a deterministic MDP and a set of deterministic policies, it is strange to define $\varphi_{Q, \Pi}$ over $\mathcal{X}$ since there may be state-actions not visited.
% The assumption can be fulfilled by appending $(x_i, R_i=0)$ to $D_\pi$ for the state $x_i$ that is not visited by $\pi$.
% \end{remark}

\begin{remark}
If two state-actions (which may be essentially similar) do not appear in a same trajectory for some policy, $d_1$ will treat them as different state-actions.
This style of aggregation seems too strict.
\end{remark}

\begin{theorem}
Under the Assumption \ref{assumption:detMDP}, Algorithm \ref{algo:exact} returns an abstraction metric that equals to $d_1$.
\end{theorem}

\begin{proof}
Since the environment (i.e., the dynamics of the MDP and the initial state) and the policies are deterministic, the (discounted) return is equal to the Q value.

By letting
\begin{equation*}
\begin{aligned}
\dfrac{\partial L(d;D)}{\partial d(x_i, x_j)} 
% & = \dfrac{\partial}{\partial d(x_i, x_j)} \bigg(
% \sum_{\pi\in\Pi} \mathbb{I}[x_i \in \mathcal{X}_\pi \text{ \& } x_j \in \mathcal{X}_\pi] \\
% & 
% \quad \quad \left(
% \mathbb{I}[R_i \neq R_j] \log d(x_i, x_j) + (1 - \mathbb{I}[R_i \neq R_j]) (1 - d(x_i, x_j))
% \right)
% \bigg)
% \\
& \propto \dfrac{\partial}{\partial d(x_i, x_j)} \bigg(
d_1(x_i, x_j) \log d(x_i, x_j) + (1-d_1(x_i, x_j)) \log (1 - d(x_i, x_j))
\bigg)
\\
& = 0,
\end{aligned}
\end{equation*}
we obtain $d(x_i, x_j) = d_1(x_i, x_j)$.

% \begin{equation*}
% - L(d;D) \propto \sum_{x_i, x_j \in \mathcal{X}} \sum_{\pi \in \Pi} \left[
% d^*(x_i, x_j) \log d(x_i, x_j) + (1-d^*(x_i, x_j)) \log (1 - d(x_i, x_j))
% \right].
% \end{equation*}

% Then, 
% $
% \dfrac{\partial L(d;D)}{\partial d(x_i, x_j)} = 0
% $
% yields 
% $d(x_i, x_j) = d^*(x_i, x_j)$.

\end{proof}

In practice, instead of learning an abstraction metric, we could learn an abstraction representation $\psi: \mathcal{X} \to \mathbb{R}^m$.
In this case, we could either solve the following optimization problem:

\begin{equation}
\begin{aligned}
    & \max_{\psi} \mathbb{E}_{(x_i, x_j, x_k) \sim D} 
    \left[ 
    \log \dfrac{1-\psi(x_i)^T \psi(x_j)}{1+\psi(x_i)^T \psi(x_j)} + \beta \log (1+\psi(x_i)^T \psi(x_k))
    \right] \\
    & s.t. ||\psi(x)|| = 1, \forall x \in \mathcal{X} \\
\end{aligned}
\end{equation}

or train a DNN to generate the abstraction metric with the abstraction representations as inputs, e.g., $F(\psi(x_1), \psi(x_2)) \in [0,1]$, where $F$ and $\psi$ are DNNs.

\begin{corollary}
Under the Assumption \ref{assumption:detMDP} and given $\Pi = \Pi_1$, Algorithm \ref{algo:exact} returns an abstraction metric of $\varphi_{Q, \Pi_0}$, and the corresponding representation preserves the value functions for any policy.
\end{corollary}

\subsection{Towards practical algorithms}

The condition for aggregation in $d_1$ is too strict and Algorithm \ref{algo:exact} requires to access the full state-action space.
Here, we provide another modified version of algorithm to alleviate these two problems.

\begin{algorithm}[H]
\label{algo:2}
\SetAlgoLined
    \KwIn {A set of deterministic policies $\Pi\subseteq \Pi_1$}
    \KwOut {An abstraction metric of $\varphi_{Q, \Pi}$}
    \ForEach{$\pi$ in $\Pi$}{
        Roll out $\pi$ till end and collect the state-actions and the returns $D_\pi = \{(x_i, R_i)\}$
        
        $D \leftarrow D \cup \{(x_i, x_j, y): (x_i, R_i) \in D_\pi, (x_j, R_j) \in D_\pi, y=\mathbb{I}[ R_i \neq R_j ]
        \}
        $
    }
    % $\beta \leftarrow |\Pi| n^2 / |D|$
    
    $d \leftarrow arg \min_{d} L(d;D)$, where \begin{equation}
    \label{eq:loss_d}
    L(d;D) = - \mathbb{E}_{(x_i, x_j, y) \sim D} 
    \left[ 
    y \log d(x_i, x_j) + (1-y) \log ( 1- d(x_i, x_j) )
    % \log \dfrac{d(x_i, x_j)}{1-d(x_i, x_j)} + \beta \log (1-d(x_i, x_k))
    \right] 
    \end{equation} 
    
    \Return{d}
\caption{Learn an abstraction representation of a Q-irrelevance abstraction}
\end{algorithm}

Similarly, we show that this algorithm outputs the following solution:

\begin{equation}
d_2(x_1, x_2) = \dfrac{\sum_{\pi \in \Pi} \mathbb{I}  [ x_1 \in \mathcal{X}_\pi \text{ \& } x_2 \in \mathcal{X}_\pi \text{ \& } Q^\pi(x_1) \neq Q^\pi(x_2) ]
}{\sum_{\pi \in \Pi} \mathbb{I}  [ x_1 \in \mathcal{X}_\pi \text{ \& } x_2 \in \mathcal{X}_\pi ]},
\end{equation}

\begin{theorem}
Under the Assumption \ref{assumption:detMDP}, Algorithm \ref{algo:2} returns $d_2$.
\end{theorem}

\begin{proof}
Similarly, by letting
\begin{equation*}
\begin{aligned}
\dfrac{\partial L(d;D)}{\partial d(x_i, x_j)} 
& = \dfrac{\partial}{\partial d(x_i, x_j)} \bigg(
\sum_{\pi\in\Pi} \mathbb{I}[x_i \in \mathcal{X}_\pi \text{ \& } x_j \in \mathcal{X}_\pi] \\
& 
\quad \quad \left(
\mathbb{I}[R_i \neq R_j] \log d(x_i, x_j) + (1 - \mathbb{I}[R_i \neq R_j]) (1 - d(x_i, x_j))
\right)
\bigg)
\\
& \propto \dfrac{\partial}{\partial d(x_i, x_j)} \bigg(
d_2(x_i, x_j) \log d(x_i, x_j) + (1-d_2(x_i, x_j)) \log (1 - d(x_i, x_j))
\bigg)
\\
& = 0,
\end{aligned}
\end{equation*}
we obtain $d(x_i, x_j) = d_2(x_i, x_j)$.

\end{proof}

\begin{lemma}[Relationship between $d_1$ and $d_2$]
Given $x_1, x_2 \in \mathcal{X}$, $d_1(x_1, x_2) \ge d_2(x_1, x_2)$.
Specifically, if $d_1(x_1, x_2) = 0$ for some $x_1, x_2 \in \mathcal{X}$, $d_2(x_1, x_2) = 0$;
if $d_2(x_1, x_2) = 1$ for some $x_1, x_2 \in \mathcal{X}$, $d_1(x_1, x_2) = 1$.
\end{lemma}

\begin{remark}[$d_2$ is the lower bound of $d_1$]
If we do not have access to the full state-action space, we construct $D$ with only the encountered state-actions. Then, we will obtain $d_2$ which is the lower bound of the abstraction metric $d_1$. Notice that $d_2$ is not a semimetric since it does not satisfy triangle inequality.
\end{remark}

\begin{remark}[Practical algorithm that incorporates DQN/Rainbow]
Further, this motivates us to use the trajectories in the replay buffer to construct $D$ and use $L(d; D)$ as the loss function to learn the approximate abstraction representation of $\varphi_{Q, \Pi}$ where $\Pi$ is the set of the deterministic policies induced by the transitions in the replay buffer.
Moreover, we use this as the auxiliary task along with a standard RL algorithm.
\end{remark}
